Benchmarking the Accuracy and Robustness of Feedback Alignment Algorithms

Backpropagation is the default algorithm for training deep neural networks due to its simplicity, efficiency and high convergence rate. However, its requirements make it impossible to be implemented in a human brain. In recent years, more biologically plausible learning methods have been proposed. Some of these methods can match backpropagation accuracy, and simultaneously provide other extra benefits such as faster training on specialized hardware (e.g., ASICs) or higher robustness against adversarial attacks. While the interest in the field is growing, there is a necessity for open-source libraries and toolkits to foster research and benchmark algorithms. In this paper, we present BioTorch, a software framework to create, train, and benchmark biologically motivated neural networks. In addition, we investigate the performance of several feedback alignment methods proposed in the literature, thereby unveiling the importance of the forward and backward weight initialization and optimizer choice. Finally, we provide a novel robustness study of these methods against state-of-the-art white and black-box adversarial attacks.

==> 3_adversarial_attacks.tex <==
%However, a big weakness currently is that these black-box attacks need to query the classifier too many times before they find adversarial examples, and their success rate is sometimes significantly lower than that of white-box attacks.
\iffalse
\textbf{FGSM:}~~One of the earliest versions of to generate an adversarial example $x^{\textrm{adv}}$ is  the Fast Gradient Sign Method  (FGSM)~\cite{goodfellow2014explaining} which updates the original image $x$, whose label is $y^*$, using the direction of the sign of the gradient w.r.t. the image as follows:
\begin{equation}
\label{eq:fgsm-attack}
x^{\textrm{adv}} = x + \epsilon \;\textrm{sign}\big(\nabla_x\,\mathcal{L}(x, y^*)\big)
\end{equation}

\textbf{PGD, APGD and TRADES:}~~The Projected Gradient Descent (PGD)~\cite{madry2017towards} is a variant of FGSM attack applied multiple times with a step size $\alpha$. That is to say:
\begin{equation}\label{eq:bmi-attack}
x^{\textrm{adv}}_0 = x,\quad\quad x^{\textrm{adv}}_{t+1} = \textrm{Clip}_{x}^{\epsilon}\bigg( x^{\textrm{adv}}_{t}  + \alpha \;\textrm{sign}\big(\nabla_x\,\mathcal{L}(x^{\textrm{adv}}_{t}, y^*)\big)\bigg)
\end{equation}
where the function $\textrm{Clip}_{x}^{\epsilon}(\cdot)$ clips its parameter to be within the $\epsilon$-ball of $x$.

\textbf{Few-Pixel:}~~Carefully designed perturbations that are even unrecognizable by human eyes can be appropriately perturbed using the one-pixel attack~\cite{su2019one} based on differential evolution. While  common adversarial attacks are constructed by perturbating all pixels with an overall constraint on the strength
of the accumulated modification (e.g., the perturbation $\epsilon$ in FGSM and the ball radius $\epsilon$ and the step size $\alpha$ in PGD), the few-pixel attack limits the number of pixels to modify without confining the strength of modification. In this paper we consider the n-pixel attack where $\textrm{n}\in\{1,2,3,4,5\}$.

\textbf{Square:}~~Without the need for the local gradient information, the square attack~\cite{andriushchenko2020square} is a score-based that is based on a randomized search scheme which selects localized square shaped updates at random positions to iteratively generate adversarial samples on the surface of the $l_{\infty}$- or $l2$-balls. This attack outperforms many more sophisticated attacks in terms of success rate and query efficiency.
\fi

==> images/robustness/whitebox/legend.tex <==
\protect\tikz \fill[bp-color] (0,1) rectangle ++ (0.5,0.05); ~~BP~~
\protect\tikz \fill[fa-color] (0,1) rectangle ++ (0.5,0.05); ~~FA~~
\protect\tikz \fill[dfa-color] (0,1) rectangle ++ (0.5,0.05); ~~DFA~~
\protect\tikz \fill[uSF-color] (0,1) rectangle ++ (0.5,0.05); ~~uSF~~
\protect\tikz \fill[brSF-color] (0,1) rectangle ++ (0.5,0.05); ~~brSF~~
\protect\tikz \fill[frSF-color] (0,1) rectangle ++ (0.5,0.05); ~~frSF
